Submolecular-scale control of phototautomerization

Many natural and artificial reactions including photosynthesis or photopolymerization are initiated by stimulating organic molecules into an excited state, which enables new reaction paths. Controlling light-matter interaction can influence this key concept of photochemistry, however, it remained a challenge to apply this strategy to control photochemical reactions at the atomic scale. Here, we profit from the extreme confinement of the electromagnetic field at the apex of a scanning tunneling microscope (STM) tip to drive and control the rate of a free-base phthalocyanine phototautomerization with submolecular precision. By tuning the laser excitation wavelength and choosing the STM tip position, we control the phototautomerization rate and the relative tautomer population. This sub-molecular optical control can be used to study any other photochemical processes.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
